PolarFly: A Cost-Effective and Flexible Low-Diameter Topology

In this paper we present PolarFly, a diameter-2 network topology based on the Erdos-Renyi family of polarity graphs from finite geometry. This is a highly scalable low-diameter topology that asymptotically reaches the Moore bound on the number of nodes for a given network degree and diameter PolarFly achieves high Moore bound efficiency even for the moderate radixes commonly seen in current and near-future routers, reaching more than 96% of the theoretical peak. It also offers more feasible router degrees than the state-of-the-art solutions, greatly adding to the selection of scalable diameter-2 networks. PolarFly enjoys many other topological properties highly relevant in practice, such as a modular design and expandability that allow incremental growth in network size without rewiring the whole network. Our evaluation shows that PolarFly outperforms competitive networks in terms of scalability, cost and performance for various traffic patterns.

==> construction_orig.tex <==
%\kldelete{\section{Erd\H os-R\'enyi Polarity Graphs}\label{sec:math_construction}}
\section{PolarFly Topology}
In this section, we discuss in detail the graph underlying the \fly layout. This mathematical description is used in the construction and for the exploitation of the graph properties.

The topology of PolarFly is an
Erd\H os-R\'enyi (ER) polarity graph, constructed using the relationship of points and lines in finite geometry. These were discovered by Erd\H os and R\'enyi \cite{erdosrenyi1962} and independently discovered by Brown \cite{brown_1966}.
% , and were independently discovered by Brown \cite{brown_1966}. 
There is a great deal of mathematical structure to these graphs, and they have been studied in depth, both in the original papers \cite{erdosrenyi1962,brown_1966} and in many other references \cite{brown_1966, bachraty_siran_2015, miller2005, parsons_1976}.

ER graphs have several useful features for network design: 
\begin{itemize}
    \item \textbf{Low diameter.} Their diameter is 2, giving a short path between any two nodes.
    \item \textbf{Scalability.}
    At the same time, they asymptotically reach the Moore bound, surpassing the scalability of all other diameter-2
    topologies. We compare to other diameter-$2$ topologies that are direct, as needed for co-packaging, and show the comparison in Figure \ref{fig:mb}.
    \item \textbf{Flexibility.} They cover a wide range of degrees,
    having degree $k=q+1$ for every prime
    power $q$. While not completely general, they meet or comes very close to the radixes of many current and near-term high-radix routers. For example, for $q=31, 47, 61$ and $127$, $ER_q$ may be applied to systems with routers of radix 32, 48, 64 and 128, with all router ports used at radix 32, 48 and 128. 
     %\item \lmcomment{triangles and elegance of design}
    
    %\lmedit{\item Do we want to mention triangles at all, at least in terms of how they contribute to the simplicity of the layout?}\klcomment{As Prof. Torsten said, "simplicity" is a slightly vague term, unless we come up with a clear measure of it. I would avoid.}\lmcomment{Perhaps I misunderstood -- I thought he was saying that the layout was unclear and apparently difficult -- without a picture.}
\end{itemize}
\begin{figure}[ht]
\begin{centering}
%
%\includegraphics[width=1.0\columnwidth]{plot_MB2___e.pdf}
\includegraphics[width=.8\columnwidth]{figs/moore_bound_comparison.pdf}
\caption{Scalability of direct diameter-2 topologies in terms of 
the optimal Moore bound.}
\label{fig:mb}
%
\end{centering}
\end{figure}

%Erd\H os-R\'enyi graphs are defined in terms of prime powers $q$.  In this paper, we discuss only odd $q$, and use graph properties specific to odd $q$ in development of the algorithm presented here. We note that the graph construction is the same for even $q$, but the layout in Section X will be different. We emphasize that it is possible to 
%, but that is out of scope for this paper.
%\klcomment{This sentence makes it look like even $q$ is a different topology. Do we need to mention it here? Construction of the graphs is same for even or odd $q$, layout is different. We can mention it then.} \kicomment{Makes sense to me - I commented this paragraph out for now} \lmcomment{I do think we should say somewhere why we are only looking at odd $q$ in this paper. I think up front in the layout section would work. Maybe a sentence before property \ref{prop:er}, noting that it applies to odd $q$ and we are going to use that.}

\subsection{Some Background on Finite Fields and Their Arithmetic}\label{sec:ff}
The construction of ER polarity graphs is based upon the arithmetic operations of finite fields. 
A field is a set having addition and multiplication, where every element has an additive inverse, and every non-zero element has a multiplicative inverse. The construction of ER polarity graphs depends especially upon the existence of multiplicative inverses. 
The set of integers mod a prime $p$ is an example of a finite field. 

Finite fields $\mathbb{F}_q$ of order $q$ exist for all prime powers $q$, and for no other integers. 
Finite fields are 
%also called Galois extension fields. They are 
fundamental to many areas in mathematics and computer science, and are discussed in detail in \cite{mceliece_1987,lidl_niederreiter_1994,gallian_2020} and in many other references. 

It is important to note that addition and multiplication operations in $\mathbb{F}_q$ are quite different from those in $\mathbb{R}$:
\begin{itemize}
\item If $q=p$ is a prime, then addition and multiplication are just modular arithmetic over $p$.
\item If $q=p^m$ is a prime power, with $m>1$, then
%the arithmetic 
addition and multiplication in $\mathbb{F}_q$ are 
%not simply modular over $q$, but instead are 
derived from modular arithmetic over an irreducible degree-$m$ polynomial over the field $\mathbb{F}_p$. For further details on arithmetic in the finite fields $\mathbb{F}_q$, see 
any of the references listed above.
%\cite{mceliece_1987}. 
\end{itemize}

We will use primes $q=p$ for the examples in this paper for simplicity, so the addition and multiplication in the dot products is just modular arithmetic over $p$. The same graph construction will hold for any prime power $q=p^m$, using the associated arithmetic of $\mathbb{F}_q$ for the dot products. 

\subsection{Geometric Intuition}\label{sec:geom_int}
%\subsubsection{Geometric Construction}
%ER graphs are based on the geometric concept of perpendicularity, or orthogonality. The \emph{dot product} is a convenient way of expressing this; two length-$n$ vectors $v$ and $w$ are orthogonal when $v\cdot w = \sum_{i=0}^n v_i w_i = 0$. 

% In general, graphs may be understood to express relationships between objects. The relationship that 
Erd\H os-R\'enyi polarity graphs express the orthogonality (or perpendicularity) between vectors, or equivalently, lines passing through the origin.  The \emph{dot product} is a convenient way of expressing this; two length-$n$ vectors $v$ and $w$ are orthogonal when $v\cdot w = \sum_{i=0}^n v_i w_i = 0$. 

Note that multiples of a vector retain the same orthogonality relationships as the original vector. So for our purposes, we may consider all multiples of a vector to be the same, and simply choose one as representative of all its multiples.

ER polarity graphs are defined by vertices that represent length-$3$ vectors over a field, and edges that exist between two vertices if the vectors they represent are orthogonal. This graph is of diameter $2$.

As an example, consider ordinary Euclidean $3$-dimensional space. The existence of $2$-hop paths between any two vectors in the corresponding graph depends upon this fact: any pair of (non-multiple) vectors has a vector to which both are orthogonal: their cross-product. The $2$-hop path linking them passes through the orthogonal vector. This is shown in Figure~\ref{fig:cp}.
\input{figs/cross_product}

 Euclidean $3$-space obviously has infinitely many lines and planes passing through the origin. However, a similar construction may be used to obtain a finite space of dimension $3$ over the finite field $\mathbb{F}_q$.
 %, the Galois field of order a prime power $q$. 
%A field is a set having addition and multiplication, where every element has an additive inverse, and every non-zero element has a multiplicative inverse. The multiplicative inverse is needed so that each line may be represented by exactly one vector, having $1$ as its first non-$0$ entry. Finite fields $\mathbb{F}_q$ of order $q$ exist for prime powers $q$, and only for those $q$. 
%These fields are called Galois extension fields. Galois fields are fundamental to many areas in mathematics and computer science, and are discussed in great detail in many references, such as \cite{g1} and \cite{g2}. \lmcomment{Tried to rewrite this so that just enough is said to be intuitively clear, and no more.}
%This construction gives a geometric space with $q^2+q+1$ lines, since any non-zero multiple of a point on the line is on the same line. This is why the multiplicative inverses of a field are needed. 
The geometric relationships are similar to those discussed above in the Euclidean case. Orthogonality is again expressed by the dot product, using the addition and multiplication from $\mathbb{F}_q$. So the construction over $\mathbb{F}_q$ also gives rise to a graph of diameter $2$, but this time the graph is finite.
 
%It is important to note that the addition and multiplication operations in $\mathbb{F}_q$ are quite different from addition and multiplication in $\mathbb{R}$. If $q=p$ is a prime, then addition and multiplication are just modular arithmetic over $p$. If $q=p^k$ is a prime power, with $p$ a prime and $k>1$, then the Galois field $\mathbb{F}_q$ has operations derived from modular arithmetic over an irreducible degree-$k$ polynomial over the field $\mathbb{F}_p$, as discussed in \cite{g1} and \cite{g2}. 
 
Because $\mathbb{F}_q$ is finite with modular arithmetic, some non-zero vectors in $\mathbb{F}_q^3$ have the interesting property that they are orthogonal to themselves, which never happens in Euclidean space. For example, consider $\mathbb{F}_3^3$, where the arithmetic operations are modular addition and multiplication$\mod 3$. The vector $[1,1,1]$ is self-orthogonal, since $[1,1,1]\cdot [1,1,1]=1+1+1=0 \mod3$. 
\subsection{Construction With Dot Products over $\mathbb{F}_q$}
ER polarity graphs are easily constructed using the set of non-zero vectors $[x,y,z] \in \mathbb{F}_q^3$ as vertices. We use left-normalized vectors as representatives of their multiplicative classes. These are vectors in which the first non-zero entry is $1$.  

For example, in $\mathbb{F}_3^3$, $[1,0,2]$ and $[0,1,0]$ are vectors in the set under consideration, but $[0,2,1]$ would not be, since its first non-zero entry is $2$. Instead, $[0,2,1]$ is multiplied by the multiplicative inverse of $2$ (mod $3$), giving its left-normalized representation: $2\cdot [0,2,1] = [0,1,2]$. The existence of multiplicative inverses in the field $\mathbb{F}_q$ assures us that each non-zero vector can be represented as a left-normalized vector.

\ER{q} is then constructed as follows:

\begin{itemize}
\item The vertices are the left-normalized vectors in $\mathbb{F}_q^3$. 
\item The edges are pairs $(v,w)$ of vertices that are orthogonal to each other.
% ; in other words, using the addition and multiplication of $\mathbb{F}_q$, the dot product of $v$ and $w$ is 0. 
\end{itemize}
Self-orthogonal vertices are distinguished from the others and are called 
\textit{quadric}. All other vertices are called \textit{non-quadrics}. Quadrics may be considered to have a self-loop, and play a special role in the construction of \fly.

We show an example of this construction in Figure \ref{fig:dpc}. There is a great deal of structure in the $ER_q$ graph, some of which can be seen there and in the graph layout in Figure~\ref{fig:clustercake_design}. We exploit this in the construction of an efficient network.
\input{figs/dotprod_construction.tex}
\subsection{Formal Construction}
%\htorcomment{everything until here is nice and really cute! We need to realize that we have probably lost 60\% of the readers of the architecture track at SC by now} \lmcomment{yeah, it's rough. I've come across this before with the math/CS crossover papers I've done. Nothing to be done about it here, this is such a math-based construction. Except explain the math as clearly as possible ... Maybe prep them for it with an up-front remark in the intro that this is math-inspired.}
\subsubsection{A Bipartite Graph  From Finite Geometry}
The projective plane $\textrm{PG}(2,q)$ is a geometric structure that arises from projecting lines and planes in three-dimensional space over $\mathbb{F}_q$ to points and lines respectively. As discussed above, projective points can be thought of as the left-normalized vectors in $\mathbb{F}_q^3$. In more formal language, each point $[a]$ in $\textrm{PG}(2,q)$ is an equivalence class of 3-tuples where $(a_1 , a_2 , a_3) \sim (b_1, b_2, b_3)$ if and only if these tuples are multiples of each other. Projective lines $(b_1: b_2:b_3)$ contain all points $[x]$ so that $b_1x_1 + b_2x_2+ b_3x_3=0$ in $\mathbb{F}_q$.  By counting such vectors, we see there are $q^2+q+1$ points in $\textrm{PG}(2,q)$. Dually, there are $q^2+q+1$ lines in $\textrm{PG}(2,q)$ as we will see. 

We will construct $\textrm{ER}_q$ graphs for any prime power $q$ using properties of points and lines in $\textrm{PG}(2,q)$.  To begin, we first build a bipartite graph $B(q)$. The vertex set of $B(q)$ is $U \cup V$  where $U$ is the set of points in $\textrm{PG}(2,q)$ and $V$ is the set of lines in $\textrm{PG}(2,q).$ There is an edge between $v \in U$ and $w\in V$ if and only if the point $v$ lies on the line $w$. 
In $\textrm{PG}(2,q)$, each point lies on $q+1$ lines, and each line contains $q+1$ points. The graph $B(q)$ has $2(q^2+q+1)$ vertices and degree $q+1.$ The graph $B(q)$ has diameter 3, which will be reduced to diameter 2 by a polarity construction in the next section.

\subsubsection{Decreasing the Diameter Using a Polarity Map}
For each point $[a]$ in $\textrm{PG}(2,q)$, the \emph{dual} $[a]^\perp$ is the line in $\textrm{PG}(2,q)$ which contains all points $(x_1, x_2, x_3)$ so that $a_1 x_1 + a_2 x_2 + a_3 x_3 =0$. Since the dual map is a bijection, this shows that $\textrm{PG}(2,q)$ contains $q^2+q+1$ lines. The dual of a line can be defined symmetrically. Notice that $([a]^\perp)^\perp =[a]$. Clearly, 
$[x]$ lies on line $[a]^\perp$ if and only if $[a]$ lies on
$[x]^\perp$. Such a bijection is also known as \textit{polarity}.

In order to decrease the diameter of $B(q)$, we use this polarity: Take $B(q)$ and glue the vertices $v \in U$ and $w \in V$ together if and only if $[w] = [v]^\perp$. That is, combine the point $[v] \in U$ and the line $[w]\in V$ together if they are duals of each other. Define \ER{q} to be the graph formed by applying this gluing process to $B(q)$. \ER{q} has $q^2+q+1$ vertices since we glued pairs of vertices in $B(q)$ together. The degree is still $q+1$, since every line passing through point $[v]$ is
glued to a point on $[v]^\perp$, but now the diameter is reduced to 2.

This construction is quite general: if a polarity map exists on a bipartite graph with $N=2n$ vertices, maximum degree $k$, and diameter $D$, it can be used to construct another graph with $n = \frac{N}{2}$ vertices, maximum degree $k$, and diameter $D-1$. 

\subsubsection{Quadric Vertices}
In a finite geometry, the point $[a]$ may lie on its own dual, the line $[a]^\perp$. When this occurs, i.e., when $a_1^2 + a_2^2 + a_3^2=0$, the vertex $[a]$ is called a \emph{quadric vertex}. In \ER{q}, there is a loop at vertex $[a]$ since $[a]$ and $[a]^\perp$ are glued together. These quadric vertices are the same as the self-orthogonal vectors discussed at the end of Section \ref{sec:geom_int}, and will be discussed further in Section \ref{sec:layout_property} in terms of the layout of the network.


%\subsubsection{Generalized Polygons/Triangles}
%\lmcomment{We might want to limit this section to generalized triangles, with attention to how they can impact the form of the network. This also speaks to odd $q$ since there are no triangles for even $q$.}
%\kicomment{The projective plane $\textrm{PG}(2,q)$ is a generalized triangle, but the ER graphs are not - what do we need to say about generalized triangles? Is it sufficient just to explain that a triangle is a 3-cycle?}
%\klcomment{I think we can just skip this subsection.}

%\subsection{Abas Graph Construction}
%\klcomment{I think we can skip Abas in this paper} \lmcomment{so just cut this section now?}
%\begin{itemize}
%    \item Exist for all degrees
%    \item vertex transitive
%\end{itemize}

%\subsubsection{Semidirect Product}

%\subsubsection{Intuition on structure, Two sets of vertices}
\subsection{Structural Properties of \topo}\label{sec:layout_property}
We make heavy use of the structure of ER graphs in the design of the network discussed in this paper. 

ER graphs \ER{q} have $N=q^2+q+1$ vertices, degree $k=q+1$, and 
diameter $D=2$. The vertex set of \ER{q} can be divided into three
disjoint subsets~\cite{parsons_1976}:
\begin{itemize}
\setlength\itemsep{.35em}
    \item \quadric{q}$\rightarrow$ set of $q+1$ quadric vertices. 
    % \quadric{q} is an independent set of 
    % $q+1$ vertices.
    
    \item \lone{q}$\rightarrow$ set of $\frac{q(q+1)}{2}$ vertices 
    adjacent to \quadric{q}. 
    % \lone{q} contains $\frac{q(q+1)}{2}$ vertices
    
    \item \ltwo{q}$\rightarrow$ set of $\frac{q(q-1)}{2}$ vertices not adjacent to 
    \quadric{q}.
\end{itemize}
The following properties used in the construction and analysis of the network were presented by Bachrat\'y and \v{S}ir{\'a}\v{n} in \cite{bachraty_siran_2015}. 

\begin{property}\cite{bachraty_siran_2015}\label{prop:er}
For every odd prime power $q$, \ER{q} has the following properties:
    \begin{enumerate}
\setlength\itemsep{.35em}
        \item 
        %\quadric{q} is an independent vertex set i.e.
        No two vertices in 
        \quadric{q} are directly 
        connected.
        Every vertex in \quadric{q} is adjacent to exactly $q$ vertices in \lone{q}.\label{prop:quad_adj}

        \item Every vertex in \lone{q} is adjacent 
        to exactly $2$ vertices in \quadric{q}, and 
        $\frac{q-1}{2}$ vertices each in \lone{q} 
        and \ltwo{q}.\label{prop:lone_adj}
        
        \item Every vertex in \ltwo{q} is adjacent 
        to exactly $\frac{q+1}{2}$ vertices each in 
        \lone{q} and \ltwo{q}.
        
        \item There is exactly one path of length two
        between every vertex pair (considering the  self-loop of the self-adjacent quadrics as an edge).
        %\footnote{Every quadric vertex $v$ is incident with a self loop which is a part of the 2-hop paths between $v$ and its neighbors.}.
        \item As a corollary, the edges incident with quadric vertices
        do not participate in any triangle. 
        Any edge incident with two non-quadric 
        vertices participates in exactly
        one triangle.
        \label{prop:path}
    \end{enumerate}
\end{property}




==> evaluation.tex <==
\section{Evaluation} 
\label{sec:eval}





==> intro_orig.tex <==

\section{Introduction}
\label{sec:intro}

High performance computing is progressing at a torrid pace. 
The recently announced Intel Ponte Vecchio GPU, based on the X$^e$HPC microarchitecture,  employs a total of 47 chiplets, and over 100 billion transistors in the aggregate across those tiles. The A0 silicon performance is providing more than 45 TFLOPS FP32 throughput, 5 TB/s memory fabric bandwidth and 2 TB/s connectivity bandwidth\cite{blythe:xehpc-pontevecchio}.
\if 0
\lmcomment{need a sentence here about how the compute is great on this but we cannot fully exploit it -- one of the CS people?}\klcomment{Rearranging back to the previous version for now.}
\fi

While raw compute power has improved very quickly over the last few years, electrical I/O is lagging behind and is fast approaching performance and power limitations.
Systems are increasingly limited by our ability to move data around -- both on chip and off chip. Power consumption in a computing package has been going up significantly over time, but at a relatively shallow trend if compared to data movement.  The power required by the interconnect is approaching, in some cases, $40\%$ to $50\%$ of the overall chip budget. These technological trends are extrapolated in Figure~\ref{fig:darpa-eri} presented at the 2019 DARPA ERI Summit \cite{darpa-eri-2019, mahajan2021co, wade2020teraphy}. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.35\textwidth]{figs/plot_power.pdf}c
    \caption{System performance is increasingly limited by data movement.
    Data points obtained from high performance CPUs, GPUs, FPGAs and ASICs}
    \label{fig:darpa-eri}
\end{figure}
\subsection{Current hardware approaches}
The industrial and academic communities are aggressively trying to increase I/O bandwidth efficiency and reducing power consumption by bringing silicon photonic connections directly into the chip, using 2.5D \cite{sipho-2.5d:Bergman} or 3D \cite{3d-multichip:Bergman} integration and deploying Multi Chip Packages (MCP)~\cite{EMIB:Mahajan}. This integration is typically defined as co-packaging. Chiplet-based technologies have emerged as a scalable approach to integrating heterogeneous electrical functionality (high-speed analog, memories, custom accelerators, etc.) inside MCPs. While silicon photonics is widely adapted in data centers,  a co-packaging approach attains a much closer level of integration and short reach connections, with the goal of reducing, or possibly eliminating altogether, electrical connections. 

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=0.25\textwidth]{figs/teraphy-hand.png}
%    \caption{An assembled TeraPHY co-packaged with an Intel Stratix10 FPGA multichip package from~\cite{wade2020teraphy, darpa-eri-2019}. \lmcomment{This figure could perhaps be cut, since it addresses only current-day state-of-the-art; hopefully the paper is relevant for a long time}}
%    \label{fig:teraphy}
%\end{figure}
Notable industrial players in this space are Ayar Labs~\cite{wade2020teraphy}, Avicena~\cite{avicena}, Teramount~\cite{teramount}, LighMatter~\cite{lightmatter}, DustPhotonics~\cite{dustphotonics}, Celestial AI~\cite{celestialai}, Axalume~\cite{axalume}, and others.
%
For example, as a part of the DARPA PIPES program, Ayar Labs has recently co-packaged a TeraPHY chiplet with an Intel Stratix 10 FPGA multichip package demonstrating 1 Terabit/sec with 5pJ/bit.
%, cf.~Figure~\ref{fig:teraphy}.
%
Another example is Avicena, who recently announced an optical interconnect based on technology from display microLEDs. The company’s LightBundle leverages microLED light sources and medical multicore fibers to create highly parallel interconnects that Avicena say can enable chip-to-chip communications at distances up to 10 meters.  Several academic groups are also evaluating novel concepts in short-reach, ultra-low-power photonics~\cite{mahajan2021co, wade2020teraphy}.

The emergence of co-packaged photonics is not only reducing power consumption and improving basic performance, but also impacting the overall system design. In Table~\ref{tab:criteria} we highlight some key aspects, such as the finer endpoint granularity and the increased number of available connections. In a conventional network, the endpoints are complete nodes with one or more processors, accelerators, memory modules, that are interconnected with a limited number of network interfaces sitting on an IO bus, typically PCI or CXL. Co-packaged photonics can be used to explore alternative designs when the network endpoints have a finer granularity: for example memory modules or processors. 
\begin{table}[htbp] 
\setlength{\tabcolsep}{6.0pt}
\centering
\footnotesize
\begin{tabular}{lcc@{}}
\toprule
%
\textbf{Network Type} & Conventional & Co-packaged Photonics \\
%
\midrule
%
End Point   & CPU + GPU + Memory & CPU or GPU or Memory \\ 
Network Links & 1-8 &   32-64 \\
Link Protocol & PCI/CXL & AIB \\
Latency & 100s nsec & 10s nsec \\
Bandwidth & 10s GB/sec & 2-4 TB/sec \\
%
\bottomrule
\end{tabular}
\caption{Conventional network setting vs.~co-packaged photonics.}
%\vspaceSQ{-1em}
\label{tab:criteria}
\end{table} 
\if 0
Figure~\ref{fig:disaggregated} outlines a novel disaggregated memory centric design where processors, GPUs and memory modules are directly connected with high-bandwidth, low-latency photonics connections. The PolarFly topology presented in this paper we explores how to expand this concept with a diameter 2 network.
%
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/disaggregated.pdf}
    \caption{An example disaggregated system that integrates CPUs and GPUs in a memory centric system}
    \label{fig:disaggregated}
\end{figure}
\fi

\if 0

\subsection{Emerging Disaggregated Systems}

\begin{itemize}
    \item Disaggregated systems around for a long time 
    \item fundamental limits are high bandwidth and low latency
    \item table of novel network
\end{itemize}

\begin{itemize}
    \item Processors getting very powerful (latest NVIDIA announcements)
    \item processors sockets are becoming IO limited: pin limitation, copper limitations, cost
    \item Photonics provide a way to get around these limitations
    \item some graph (DARPA Gordon Keeler)
    \item some recent results on photonics
    \item implication on system architecture/disaggregated systems
    \item figure of disaggregated system
    \item table that summarizes differences with current systems
     \item Novel view to the problem with different point of view of disaggregated systems, where endpoints are no longer processing nodes
\end{itemize}
\subsection{Competitive networks \lmcomment{or Prior Work}}

\fi





\if 0
%
2) Impact on network design - design constraints (only direct networks, need for very specific degrees AND network sizes), need for growth/modularity, full global all-to-all BW
%
\fi

\subsection{Networks approaching the Moore bound}

With co-packaged optical IO modules, each element --compute, acceleration, memory or storage, becomes a first class citizen of a highly scalable network. In this novel system design, to support good application-level performance it becomes critical that the network fabric provides low latency communication, high bandwidth and extreme scalability. 
\cite{network-disaggregation:Gao}

Slim Fly~\cite{besta2014slim} was the first topology that explicitly optimized its
structure towards the Moore bound~\cite{comb_wiki_degdiam_general}, an upper bound
on the number of vertices in a graph with given diameter and for a given maximal
degree. By fixing its diameter to $2$, Slim Fly was able to minimize construction
cost and power consumption, since the number of routers and thus buffers and ports
was smallest for a given endpoint count. Simultaneously, it also ensured
low latency and high bandwidth. %\kicomment{I've seen SlimFly in some places -- we should check this} \lmcomment{Everywhere in the text it says "Slim Fly", but in a couple of figures, it says "SlimFly".}



However, Slim Fly has several issues with respect to practical layout and
deployment. First, the number of feasible configurations/topological constructions is limited, and it is not competitive with commercially available products. Second, there are no results in the literature to address network re-configurability and expansion. This is
a matter of great importance in real-world scenarios, where data centers increase the size of a compute center gradually over time, but without being forced to rewire and re-layout the whole interconnect.
%
Finally, while Slim Fly came with a proposal on how to deploy it as a rack-level
interconnect, it is not clear how to adapt it to upcoming co-packaged
optical designs.

\if 0
%
3) Recent low-diameter networks such as Slim Fly pushed the margin in terms of
reducing cost and power while keeping high performance and resilience.
We explore it as a potential topology to build scalable co-packaged networks.
However, its practical applicability is limited because:
%
\begin{itemize}
%    \item Few design points (degrees for which topologies exist)
    \item Lack of flexibility - need to rewire entire network to add few extra nodes
    \item Low injection bandwidth for systems with overprovisioned degrees (what to do with empty ports).
%    \item Complex Layout - what consequences does this have? \maciej{This is I think not worse than the ER graphs, TBH}
\end{itemize} 
%
\fi

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/feasible_degrees.pdf}
    \caption{Design space of feasible degrees~(network radixes) for \fly and Slim Fly. Asymptotically, there are 50\% more \fly feasible degrees than what Slim Fly offers.}
    \label{fig:feasible}
\end{figure}



\subsection{Contributions}
To address the above issues, we propose \flyN{}: a diameter-2 network topology that is asymptotically optimal with respect to the Moore bound. \fly is based on 
%a class of
%degree-diameter 
%graphs called
Erd\H os-R\'enyi polarity quotient graphs. %, which %overcome Slim Fly limitations. 

\fly provides the following contributions:
\begin{itemize}
\item \fly comes with a \emph{larger
number of feasible designs}, unlike the MMS graphs that underlie Slim Fly~\cite{besta2014slim}, as shown in Figure~\ref{fig:feasible}.
Asymptotically, \fly{} offers 50\% more configurations that can be constructed, without much overlap with the design space of Slim Fly.  This is especially \emph{beneficial for co-packaged chipsets}, where the network radix is fixed.
\item 
%Importantly, 
\fly can be constructed
%on nodes with a port count of \lmcomment{
from routers having radix at --or close to, powers of $2$. In particular, one can construct instances of \fly supporting radixes $32, 48, 62$ (just less than $64$), and $128$, \emph{making the network design more practical for HW implementations}.
\item \fly has a surprisingly elegant construction that allows \emph{modularity and expansion}. Specifically, the network can be decomposed into groups of nodes, all but one of which is a fan-out of triangles, to which new node groups may be added incrementally.
\item \fly
%enjoys another advantageous topological property: it 
is asymptotically optimal in terms of the Moore bound, while Slim Fly reaches only $8/9$. Hence, \fly
%is scalable 
\emph{asymptotically supports as many routers as possible} for the router degree and the diameter $2$, and offers \emph{reductions in construction costs} of up to 20\%.
\end{itemize}
Our evaluation shows that \fly{} is performance and cost competitive with other network topologies, including Slim Fly, Dragonfly, and Fat Tree.
%Specifically, t
Thanks to its compact layout, \fly{} achieves very high saturation under random traffic with low latency, for both minimal and for non-minimal adaptive routing. Moreover, under adversarial permutation patterns, \fly{} saturates between $50\%$ and $66\%$, outperforming Slim Fly and Dragonfly, and approaching the non-blocking Fat Tree.





\if 0
%
\subsection{Contributions}
\begin{itemize}
   
    \item We present a new compact topology called PolarFly, based on polarity graphs and finite field geometry. The paper provides a detailed description of rather sophisticated the mathematical construction that is composed of three main steps (list steps) 
    \item Polarfly enjoyes many interesting topological properties: asymptotically optimal wrt Moore's bound, slimfly is only 8/9, many constructions (count vs slimfly). It also has many constructions for degrees that are relevant for existing and foreseeable routing architectures. For exampl there are (number) x constructions for degrees (range). 
    \item PF is synergistic wrt Slimfly, by addressing a key problem the sparsity of constructions. Kartik's figure.
    \item the fact convergence rate makes (numbers) make it an ideal candidate for system design
    \item The topology has a surprising elegant construction that allows partitions and expansions
    \item The experimental evaluation confirms that, thanks to the compact layout PF gets very high saturation under random traffic with low latency both minimal and UGAL.
    \item Under permutation patterns, PF delivers between $50\%$ and $66\%$, novel concept of mapping, where optimality is not reached with adjacency,
    \item novel concept of locality for permutation patterns with based on non-adjacency. Possibility of multi-phase mappings with predictable high performance
    \item partitionabiliy numbers and considerations
    \item nice visualization
\end{itemize}

\begin{itemize}
    \item Cover more all degrees. They complement Slim Fly 
        by enhancing the design space of scalable algebraic graphs.
    \item Are expandable - further racks can be added on empty ports without affecting performance.
    \item Are flexible - they cover all the needed degrees WHILE ALSO being able to deliver full global bandwidth if fewer nodes are used \maciej{is this really the case?}\klcomment{I think it could be "they cover 
    several needed degrees"}.
\end{itemize}
%
\fi



\if 0

The proposed graphs provide even better scalability than Slimfly (MMS graphs), 
asymptotically reaching the Moore bound for diameter-2.
\htorcomment{I'd be careful to over-emphasize on this, it's less than 10\% more nodes at the end - for practitioners not too relevant}

\fi


\if 0

4) We restrict the discussion to diameter-2 topologies - higher ingestion
bandwidth for given router radix \htorcomment{not sure what that means - bandwidth is adjustable in all topos for cost?}, lower latency, scalable topologies that can support
several thousands of nodes with few tens of ports. Diameter-3 (and higher) as well
as diameter-2 indirect do not satisfy the needed constraints.

\fi




 

==> layout_old.tex <==
\section{Network Design via Erd\H os-R\'enyi Graphs}
\subsection{Layout and Modularity}\label{sec:layout}
%\lkcomment{$ER(q)$ or $ER_q$? Again, we should be consistent. I would vote for $ER_q$ as this is a more math-y topic and this notation seems more in use in the math communtity.}
%\klcomment{I am fine with either. We can change the definition in sc22-diam2.tex.} \lmcomment{Done. We can change it back if we hate it.}
Topologies derived from multiple generators, such as Slimfly~\cite{} 
or Bundlefly~\cite{}, 
are naturally partitioned into hierarchical subsets (based
on different generators) comprising blades or racks in
the system.
% naturally exhibit a modular structure
% that can be easily partitioned into multiple racks. 
However, \fly is derived from polarity quotient graphs of 
finite projective planes. Hence, uniform hierarchical 
structures required for a layout
are not trivially available from the construction. 
\lkcomment{In order to back this up, we'd need to develop the 
math section a lot more. Is there an easier way to say this?}
In this section, we use the properties of \ER{q}
to obtain a simple and modular 
 layout for \fly~(\ref{sec:layout_property}).
For brevity, we only discuss \ER{q} for odd $q$ (i.e. even 
router radix) as even prime powers $q=2^i$ are sparse in the set
of all prime powers. However, layout for even $q$ is similarly
modular and extensible. 

Based on the properties of the $ER_q$ graphs discussed in Section \ref{sec:layout_property}, we propose Algorithm~\ref{alg:racks} to arrange the routers 
in \fly into $q+1$ racks that 
correspond to vertex \textit{clusters} in \ER{q}. 
We use the terms \textit{racks} and \textit{clusters} interchangeably.
\begin{algorithm}[h]
    \caption{Arranging \fly routers into racks}
    \label{alg:racks}
    \begin{algorithmic}[1]
        \Statex{\ER{q}$\leftarrow$ ER Graph of max degree $q+1$}
        \State{Initialize clusters (racks) $C_0, C_1 ... C_q\leftarrow \phi$}
        \State{Add quadrics \quadric{q} to $C_0$}
        \State{Select an arbitrary quadric $v\in W(q)$}
        \ForEach{vertex $u$ adjacent to $v$}
            \State{Add $u$ to an empty cluster $C_i$}
            \State{Add all non-quadric neighbors of $u$ to $C_i$}\label{line:add_neigh}
        \EndForEach
    \end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
%
\includegraphics[width=1.0\textwidth]{ER.pdf}
\caption{Layout and expand methods.\klcomment{Layout needs to be elaborated 
further. In method 1, we can connect each vertex 
in $C_0$ to its replica in $C_0'$ as well. We also
need to add the width of dashed links.}}
\label{fig:expand}
\end{figure*}

\klcomment{We can choose to keep or remove
the proofs for the following claims.
Adding mostly proof sketches for now.
The Lemma environment is creating strange indexing with section numbers.}
\lmcomment{Can we put any proofs in the appendix?}
\klcomment{We can't. The Artifact appendix is auto
generated from the form that we fill on SC portal.
We are not allowed to add appendices to the submission before acceptance.}
\begin{claim}\label{claim:assign1}
Algorithm~\ref{alg:racks} adds every vertex in \ER{q} to at least one cluster.
\end{claim}
\lmcomment{Do you mean "Algorithm~\ref{alg:racks} adds every vertex in \ER{q} to at least one cluster."?}\klcomment{Thanks, fixed}
\begin{proof}
Each vertex is
at most $2$-hops away from the selected quadric $v$, and algorithm~\ref{alg:racks} assigns clusters 
to $W(q)$ and all non-quadrics at shortest distance $\leq2$ from $v$.
\end{proof}
\begin{claim}
Algorithm~\ref{alg:racks} adds every vertex in \ER{q} to exactly one cluster.
\end{claim}
\lmcomment{Do you mean "Algorithm~\ref{alg:racks} adds every vertex in \ER{q} to at most one cluster."?}
\begin{proof}
This is clearly true for quadrics that are added to $C_0$.
From property~\ref{prop:er}.\ref{prop:path},
we can say that the vertices adjacent to $v$ 
are independent and do not have any common neighbor
other than $v$.
Hence, any non-quadric vertex is added to at 
most one cluster.
This combined with the claim~\ref{claim:assign1} shows that
every vertex is added to exactly one cluster.
\end{proof}
\kicomment{could we combine these claims into one?} \lmcomment{I think we should.}

\subsection{Intra-rack Layout}\label{sec:layout_intra}
\klcomment{Add figure references
as and when available.}
Let $G_i$ denote the subgraph induced by vertices 
in cluster $C_i$. We analyze the structure of
$G_i$ to derive intra-rack layout and wiring for \flyN. 
Note that since quadric vertices are independent,
there are no edges in $G_0$. 

Consider an arbitrary cluster $C_{i\mid i> 0}$ 
that contains a neighbor $u$ of the selected quadric
$v$~(algorithm~\ref{alg:racks}).
% Let $C_i$ contain vertex $u$ that is a neighbor of
% the selected quadric $v$ (algorithm~\ref{alg:racks}). 
All $q-1$ non-quadric neighbors 
of $u$ are in $C_i$. Hence, $\abs{C_i}=q$,
and there is an edge between $u$ and all other
vertices in $C_i$. We refer to $u$ as the \textit{center} of $C_i$.

Let $w\in C_i$ be a non-quadric neighbor of the
center $u$. By property~\ref{prop:er}.\ref{prop:path}, 
the edge $(u,w)$ is contained in exactly one triangle in $G_i$.
% In other words, every vertex in $C_i\setminus \{u\}$ is adjacent to $u$ and exactly one more
% vertex in $C_i$. 
Hence, $G_i$ consists of exactly 
$\frac{q-1}{2}$ edge disjoint
triangles, each of which contains $u$. 
Visually, $G_i$ has a fan-like structure
with each triangle being a fanblade and $u$
being the center of the fan\footnote{For even prime
power $q$, each cluster $C_{i\mid 0<i\leq q+1}$ induces a star graph with $\abs{C_i}=q$.
$C_0$ consists of a single node which is adjacent to
the center of every star.}.

We note that \fly has a much simpler intra-rack layout 
compared to Slimfly. Moreover, the \textit{fan-like 
layout for \fly is generalizable to any odd prime power $q$},
unlike Slimfly where generator sets and consequently,
the intra-rack layout changes significantly with $q$.
In section~\ref{sec:extensible}, we show that
this generalizability allows \fly to expand 
incrementally without rewiring the entire system.

\subsection{Inter-rack Layout}\label{sec:layout_inter}
There are two types of racks in \fly - one 
quadric rack $C_0$ and $q$ non-quadric
racks $\{C_1, ... C_q\}$. In this section,
we describe the connectivity between two racks.
For ease of notation, we use \lone{q,C_i} and 
\ltwo{q,C_i} to denote vertices of $C_i$ in 
\lone{q} and \ltwo{q} subsets, respectively~(sec.\ref{sec:layout_property}).

\begin{claim}\label{claim:C0_Ci}
For every cluster $C_{i\mid i>0}$:
\begin{enumerate}
    \item Every vertex in \lone{q,C_i} is 
    adjacent to exactly two vertices in 
    $C_0$.\label{claim:C0_Ci_1}
    \item There are exactly $q+1$ links 
between $C_i$ and $C_0$.\label{claim:C0_Ci_2}
    \item Every quadric in $C_0$ 
is adjacent to exactly one vertex in $C_i$.\label{claim:C0_Ci_3}
\end{enumerate} 
\end{claim}
\begin{proof}
Claim~\ref{claim:C0_Ci}.\ref{claim:C0_Ci_1} follows directly from property~\ref{prop:er}.\ref{prop:lone_adj}.
$C_i$ has $\frac{q+1}{2}$ vertices from \lone{q} - the center 
vertex and its $\frac{q-1}{2}$ neighbors in \lone{q}. Hence, 
there are $q+1$ edges between $C_i$ and $C_0$.

Since there is an average of $1$ link to $C_i$ per quadric,
to prove claim~\ref{claim:C0_Ci}.\ref{claim:C0_Ci_3}, it is 
sufficient to show that no quadric is adjacent to more than 
one vertex in $C_i$.
Let $v\in W(q)$ be adjacent to multiple vertices in $C_i$.
Either $v$ lies in a triangle or there are multiple
$2$-hop paths between $v$ and the center of $C_i$.
This contradicts property~\ref{prop:er}.\ref{prop:path}.
\end{proof}

\begin{claim}\label{claim:Ci_Cj}
Let $u_i$ denote the center of cluster $C_i$ for
any $0<i\leq q$.
For every $0<i,j\leq q$ where $i\neq j$:
\begin{enumerate}
    \item Every vertex in \ltwo{q,C_i} is adjacent
    to exactly one vertex in $C_j$.\label{claim:Ci_Cj_1}
    \item There is a set of $q-2$ independent edges between $C_i$ and $C_j$.
    \label{claim:Ci_Cj_2}
    \item There exists a vertex $u'\in$\lone{q,C_i}$\setminus \{u_i\}$ 
    such that every vertex in \lone{q,C_i}$\setminus\{u', u_i\}$ is adjacent
    to exactly one vertex in $C_j$, and
    $u'$ is not adjacent to $C_j$. \label{claim:Ci_Cj_3}
    \label{claim:Ci_Cj_4}
\end{enumerate}
\end{claim}
\begin{proof}
For a vertex $w\in$\lone{q,C_i}$\cup$\ltwo{q,C_i}$\setminus\{u_i\}$, let
$S(w)$ denote the set of edges between $w$ and all
clusters other than $C_i$ and $C_0$. 
If $w\in$\lone{q,C_i}, then $\abs{S(w)}=q-3$, else if 
$w\in$\ltwo{q,C_i}, then $\abs{S(w)}=k-1$. \kicomment{What is k here?}
Moreover, every edge in $S(w)$ must connect 
$w$ to a unique cluster, otherwise there will be
multiple 2-hop paths from $w$ to the center of a cluster. 
This proves claim~\ref{claim:Ci_Cj}.\ref{claim:Ci_Cj_1}.

We give a brief proof sketch for 
claim~\ref{claim:Ci_Cj}.\ref{claim:Ci_Cj_2}
and skip the details for brevity.
Adding $\abs{S(w)}$ for all vertices $w\in C_i$,
we see that there are $(q-1)(q-2)$ edges between 
$C_i$ and other non-quadric clusters. If 
claim~\ref{claim:Ci_Cj}.\ref{claim:Ci_Cj_2}
is false, then there exists a non-quadric
vertex at least $3$-hops away from the center $u_i$. 
This is a contradiction since \ER{q} has a diameter of $2$.

From claims~\ref{claim:Ci_Cj}.\ref{claim:Ci_Cj_1}
and \ref{claim:Ci_Cj}.\ref{claim:Ci_Cj_2}, we see that there
are $(q-3)/2$ independent edges between \lone{q,C_i}
and $C_j$. None of these edges are incident on $u_i$ and $\abs{\lone{q,C_i}\setminus\{u_i\}}=\frac{q-1}{2}$. 
Hence, there must be exactly one $u'\in$\lone{q,C_i}$\setminus\{u_i\}$
which is not adjacent to $C_i$.
$u'$ can be identified easily as it shares a common quadric
neighbor with center $u_j$.
\end{proof}
\kicomment{Is there a way of condensing/simplifying Claims 3 and 4? Or to give a summary of the main ideas before writing them formally? Maybe the pictures will help with this.}
Claims~\ref{claim:C0_Ci} and \ref{claim:Ci_Cj}
show that there are $\mathcal{O}(q)$ independent links
between any two racks, that can be \textit{bundled} into
cost-effective solutions such as a single multi-core fiber~\ref{}.
% For any pair of non-quadric
% clusters, these links connect unique routers 
% in the corresponding racks.
% \klcomment{Write something about how the 
% connectivity can be established with shufflers/swizzlers easily.}
% \subsection{ER Graphs}
% \klcomment{Only for even degrees (odd $q$)}
%     \begin{itemize}
%         \item Clusters $\leftrightarrow$ racks
%         \item $C_0 \leftrightarrow C_i$ connections
%         \item $C_i \leftrightarrow C_j$ connections
%         \item can be bundled
%     \end{itemize} 

% \subsection{Abas Graphs}
% \klcomment{TODO}


==> test.tex <==
\newpage
{\color{red}
\if0
\begin{property}[Multiple Triangle Connectivity]\label{prop:mult_tris}
A non-quadric cluster triplet has this property if it is joined by more than one triangle.
\end{property}
\begin{lemma}\label{lemma:clustertriplets_dualtriangles_test4}
If there exists some non-quadric cluster $X$ such that no non-quadric cluster triplet that includes $X$ has Multiple Triangle Connectivity, then no non-quadric cluster triplet has Multiple Triangle Connectivity.
\end{lemma}
\fi
\if0
\begin{lemma}\label{lemma:clustertriplets_dualtriangles_orig}
ORIGINAL: If there exists any non-quadric cluster triplet joined by more than one triangle, then every non-quadric cluster pair is part of some triplet joined by more than one triangle.
\end{lemma}
\begin{lemma}\label{lemma:clustertriplets_dualtriangles_test3}
If there exists any non-quadric cluster $X$ having the property that no triple containing $X$ is joined by more than one triangle, then every non-quadric cluster triple is joined by no more than one triangle.
\end{lemma}
\begin{lemma}\label{lemma:clustertriplets_dualtriangles_test}
If there exists any non-quadric cluster triplet joined by more than one triangle, then every non-quadric cluster is part of some triplet joined by more than one triangle.
\end{lemma}
\fi
\begin{property}[Unique Triangle Connectivity]\label{prop:non_mult_tris}
A non-quadric cluster triplet has this property if it is joined by no more than one triangle.
\end{property}
\begin{lemma}\label{lemma:clustertriplets_dualtriangles_test4}
If there exists some non-quadric cluster $X$ such that every non-quadric cluster triplet that includes $X$ has Unique Triangle Connectivity, then all non-quadric cluster triplets have Unique Triangle Connectivity.
\end{lemma}
\begin{proof}
    Let $w$ be the starter quadric, and let $X$ be a cluster having center $x_c$ with Unique Triangle Connectivity.
    
    Assume that there exists a non-quadric cluster triplet ($D$, $E$, $F$) that does not have Unique Triangle Connectivity. We will show a contradiction.
    
    ($D$, $E$, $F$) has centers $d_c$, $e_c$ and $f_c$  and is joined by two distinct triangles $(d_0, e_0, f_0)$ and $(d_1, e_1, f_1)$.
    Let $Y\neq X$ be an arbitrary cluster with center $y_c$. 
    By Theorem~\ref{th:aut_w_path}, there is an automorphism $\theta$ of $ER_q$ so that $\theta(w)=w$, $\theta(d_c)=x_c$, and $\theta(e_c)=y_c$. 
    
    Any automorphism of $ER_q$ preserves edges, so $\theta(f_c)$ is connected to $\theta(w)=w$, making $\theta(f_c)$ the center of some cluster $Z$. Again, $\theta$ preserves edges, so two distinct triangles $(\theta(d_0), \theta(e_0), \theta(f_0))$ and $(\theta(d_1), \theta(e_1), \theta(f_1))$ link $X$, $Y$ and $Z$.
    
    $X$ has Unique Triangle Connectivity, so $Z$ must be one of $X$ or $Y$. But then one of the edges of $(\theta(d_0), \theta(e_0), \theta(f_0))$ is entirely internal to that cluster. That edge $(a,b)$ will be on a triangle entirely internal to that cluster, as well as on $(\theta(d_0), \theta(e_0), \theta(f_0))$, giving two length-$2$ paths from $a$ to $b$, which can not occur.
\end{proof}
}
